Revisiting DNN Training for Intermittently-Powered Energy-Harvesting Micro-Computers

The deployment of Deep Neural Networks in energy-constrained environments, such as Energy Harvesting Wireless Sensor Networks, presents unique challenges, primarily due to the intermittent nature of power availability. To address these challenges, this study introduces and evaluates a novel training methodology tailored for DNNs operating within such contexts. In particular, we propose a dynamic dropout technique that adapts to both the architecture of the device and the variability in energy availability inherent in energy harvesting scenarios. Our proposed approach leverages a device model that incorporates specific parameters of the network architecture and the energy harvesting profile to optimize dropout rates dynamically during the training phase. By modulating the network's training process based on predicted energy availability, our method not only conserves energy but also ensures sustained learning and inference capabilities under power constraints. Our preliminary results demonstrate that this strategy provides 6 to 22 percent accuracy improvements compared to the state of the art with less than 5 percent additional compute. This paper details the development of the device model, describes the integration of energy profiles with intermittency aware dropout and quantization algorithms, and presents a comprehensive evaluation of the proposed approach using real-world energy harvesting data.

==> Algos/CkptGeMM.tex <==
\begin{algorithm}[H]
\caption{Implementing Depth-wise Separable Convolution - DWSConv2D() using CONV1D()}
\begin{algorithmic}[1]
\Function{DWSepConv2D}{$inputMatrix$, $DWsKernels$, $PtWsKernel$, $outputMatrix$}
    \State Initialize $DWsOutput$ with zero values, same shape as $inputMatrix$
    \State \# Depth-wise Separable (DWs) convolution
    \For{$c \gets 0$ \textbf{to} $channels(inputMatrix) - 1$}
        \State \# Apply 1D convolution along rows
        \For{$i \gets 0$ \textbf{to} $rows(inputMatrix[c]) - 1$}
            \State \Call{conv1D}{$inputMatrix[c][i, :]$, $DWsKernels[c][0, :]$, $DWsOutput[c][i, :]$}
        \EndFor
        \State \# Apply 1D convolution along columns
        \For{$j \gets 0$ \textbf{to} $cols(DWsOutput[c]) - 1$}
            \State \Call{conv1D}{$DWsOutput[c][:, j]$, $DWsKernels[c][:, 0]$, $DWsOutput[c][:, j]$}
        \EndFor
    \EndFor
    \State \# Point-wise (PtWs) convolution
    \State Initialize $finalOutput$ with zero values, with shape [rows($DWsOutput$), cols($DWsOutput$), channels($PtWsKernel$)]
    \For{$i \gets 0$ \textbf{to} $rows(DWsOutput) - 1$}
        \For{$j \gets 0$ \textbf{to} $cols(DWsOutput) - 1$}
            \For{$k \gets 0$ \textbf{to} $channels(PtWsKernel) - 1$}
                \State Initialize $PtWsSum \gets 0$
                \For{$c \gets 0$ \textbf{to} $channels(DWsOutput) - 1$}
                    \State $PtWsSum \gets PtWsSum + DWsOutput[c][i][j] \times PtWsKernel[c][k]$
                \EndFor
                \State $finalOutput[i][j][k] \gets PtWsSum$
            \EndFor
        \EndFor
    \EndFor
    \State \Return $finalOutput$
\EndFunction
\end{algorithmic}
\label{conv1D2conv2D}
\end{algorithm}


==> Algos/DynFit.tex <==
% \documentclass{article}
% \usepackage{algorithm}
% \usepackage{algpseudocode}
% \usepackage{amsmath}

% \begin{document}

\begin{algorithm}[ht]
\caption{DynFit Optimization Algorithm}
\begin{algorithmic}[1]
    \State \textbf{Input:} Training data \( (\mathbf{X}, \mathbf{\hat{Y}}) \), initial weights \( \mathbf{W}^{(0)} \), initial dropout rates \( \mathbf{d}^{(0)} \), initial quantization levels \( \mathbf{q}^{(0)} \), initial QuantaTask sizes \( \boldsymbol{\ell}^{(0)} \), energy budget \( E_b \), hyperparameters \( \lambda_1, \lambda_2, \alpha_q, \alpha_d, d_{\max} \), maximum iterations \( T_{\text{max}} \)
    \State \textbf{Output:} Optimized weights \( \mathbf{W} \), dropout rates \( \mathbf{d} \), quantization levels \( \mathbf{q} \), and QuantaTask sizes \( \boldsymbol{\ell} \)
    
    \State \textbf{Initialization:} Set \( t = 0 \) and initialize \( \mathbf{W}^{(0)}, \mathbf{d}^{(0)}, \mathbf{q}^{(0)}, \boldsymbol{\ell}^{(0)} \)

    \While{ \( t < T_{\text{max}} \)}
        \State \textbf{Optimize Weights \( \mathbf{W} \)}:
        \For{each batch in training data}
            \State Apply dropout mask based on \( \mathbf{d}^{(t)} \)
            \State Quantize weights and activations to \( q_j^{(t)} \) bits
            \State Compute predictions \( \mathbf{Y} \) and loss \( \mathcal{L} \)
            \State Update weights using SGD
        \EndFor
        \State \textbf{Optimize Dropout Rates \( \mathbf{d} \)}:
        \For{each neuron \( i \)}
            \State Compute gradient of objective with respect to \( d_i \)
            \State Update \( d_i \) using projected gradient descent
        \EndFor
        \State \textbf{Optimize Quantization Levels \( \mathbf{q} \)}:
        \For{each parameter \( j \)}
            \State Evaluate objective for each \( q_j \in \mathcal{Q} \)
            \State Select \( q_j^{(t+1)} \) minimizing the objective
        \EndFor
        \State \textbf{Optimize QuantaTask Sizes \( \boldsymbol{\ell} \)}:
        \For{each QuantaTask \( k \)}
            \State Compute maximum feasible size
            \State Set \( \ell_k^{(t+1)} \)
        \EndFor
        \State Update iteration \( t = t + 1 \)
    \EndWhile
    \State \textbf{Return} optimized \( \mathbf{W}, \mathbf{d}, \mathbf{q}, \boldsymbol{\ell} \)
\end{algorithmic}
\end{algorithm}

%\end{document}


==> Algos/DynInferAlgo.tex <==
\begin{algorithm}
\caption{Energy-Aware Priority Scheduling Algorithm}
\begin{algorithmic}[1]
\Require Set of tasks $\mathcal{T} = \{ T_1, T_2, \dots, T_N \}$ with parameters $E_i$, $\tau_i$, $p_i$, $D_i$, $c_i$; Energy availability function $E_b(t)$
\Ensure Schedule $\{ s_i, x_i \}$ for tasks
\State Initialize current time $t \leftarrow 0$
\While{there are unscheduled tasks in $\mathcal{T}$}
    \State Update available energy $E_b(t)$ from DynAgent
    \State Identify schedulable tasks $\mathcal{C} \subseteq \mathcal{T}$ where for each $T_i \in \mathcal{C}$:
    \begin{itemize}
        \item All predecessor tasks are completed
        \item $t + \tau_i \leq D_i$ \hfill \textit{// Deadline constraint}
        \item $E_i \leq E_b(t)$ \hfill \textit{// Energy constraint}
        \item Resource constraints are satisfied
    \end{itemize}
    \If{$\mathcal{C}$ is not empty}
        \For{each task $T_i$ in $\mathcal{C}$}
            \State Compute effective priority:
            \[
            P_i^{\text{eff}} = \frac{p_i}{E_i} \times \phi_i
            \]
            where $\phi_i = \left( 1 + \frac{D_{\max} - D_i}{D_{\max}} \right) \times c_i$
        \EndFor
        \State Select task $T_k$ with the highest $P_i^{\text{eff}}$
        \State Schedule task $T_k$: set $s_k \leftarrow t$, $x_k \leftarrow 1$
        \State Update available energy: $E_b(t) \leftarrow E_b(t) - E_k$
        \State Update current time: $t \leftarrow t + \tau_k$
    \Else
        \State Wait until energy is harvested or tasks become schedulable
        \State Increment time $t \leftarrow t + \Delta t$
    \EndIf
\EndWhile
\end{algorithmic}
\end{algorithm}

==> Algos/MADD1D2D2DDWS.tex <==
\begin{algorithm}[H]
\caption{From CONV1D to Depthwise Separable CONV2D}
\begin{algorithmic}[1]
\STATE \textbf{Function} MADD($inputA$, $inputB$, \&$out$): \# Multiply-Accumulate
\STATE \quad $out \leftarrow out + inputA \times inputB$

\STATE \textbf{Function} CONV1D($inputA$, $inputB$, $out$): \# 1D Convolution using MADD
\STATE \quad \textbf{for} $i \leftarrow 0$ \textbf{to} $|inputA| - |inputB|$
\STATE \quad \quad \textbf{for} $j \leftarrow 0$ \textbf{to} $|inputB| - 1$
\STATE \quad \quad \quad MADD($inputA[i+j]$, $inputB[j]$, $out[i]$)

\STATE \textbf{Function} CONV2D($inputA$, $inputB$, $out$): \# Extend CONV1D to 2D
\STATE \quad \textbf{for} $i \leftarrow 0$ \textbf{to} $rows(inputA) - rows(inputB)$
\STATE \quad \quad \textbf{for} $j \leftarrow 0$ \textbf{to} $cols(inputA) - cols(inputB)$
\STATE \quad \quad \quad \textbf{for} $k \leftarrow 0$ \textbf{to} $rows(inputB) - 1$
\STATE \quad \quad \quad \quad \textbf{for} $l \leftarrow 0$ \textbf{to} $cols(inputB) - 1$
\STATE \quad \quad \quad \quad \quad MADD($inputA[i+k][j+l]$, $inputB[k][l]$, $out[i][j]$)

\STATE \textbf{Function} DepthwiseSeparableConv2D($inputA$, $depthwiseKernels$, $pointwiseKernel$, $out$): \# Depthwise and Pointwise
\STATE \quad \textbf{for} $c \leftarrow 0$ \textbf{to} $channels(inputA)$
\STATE \quad \quad CONV2D($inputA[c]$, $depthwiseKernels[c]$, $out[c]$) \# Depthwise convolution
\STATE \quad \textbf{for} $i \leftarrow 0$ \textbf{to} $rows(out) - 1$
\STATE \quad \quad \textbf{for} $j \leftarrow 0$ \textbf{to} $cols(out) - 1$
\STATE \quad \quad \quad \textbf{for} $k \leftarrow 0$ \textbf{to} $channels(out) - 1$
\STATE \quad \quad \quad \quad MADD($out[k][i][j]$, $pointwiseKernel[k]$, $finalOut[i][j]$) \# Pointwise convolution
\end{algorithmic}
\end{algorithm}

==> Algos/conv1Dto2D.tex <==
\begin{algorithm}[h]
%\caption{Implementing Depth-wise Separable Convolution - DWSConv2D() using CONV1D ()}
\begin{algorithmic}[1]
\STATE \textbf{Function} DWSepConv2D($inputMatrix$, $DWsKernels$, $PtWsKernel$, $outputMatrix$):
\STATE \quad Initialize $DWsOutput$ with zero values, same shape as $inputMatrix$
\STATE \quad \# Depth-wise Separable (DWs) convolution
\STATE \quad \textbf{for} $c \leftarrow 0$ \textbf{to} $channels(inputMatrix) - 1$:
\STATE \quad \quad CONV2D($inputMatrix[c]$, $DWsKernels[c]$, $DWsOutput[c]$)
\STATE \quad \# Point-wise (PtWs) convolution
\STATE \quad Initialize $finalOutput$ with zero values, with shape [rows($DWsOutput$), cols($DWsOutput$), channels($PtWsKernel$)]
\STATE \quad \textbf{for} $i \leftarrow 0$ \textbf{to} $rows(DWsOutput) - 1$:
\STATE \quad \quad \textbf{for} $j \leftarrow 0$ \textbf{to} $cols(DWsOutput) - 1$:
\STATE \quad \quad \quad \textbf{for} $k \leftarrow 0$ \textbf{to} $channels(PtWsKernel) - 1$:
\STATE \quad \quad \quad \quad Initialize $PtWsSum \leftarrow 0$
\STATE \quad \quad \quad \quad \textbf{for} $c \leftarrow 0$ \textbf{to} $channels(DWsOutput) - 1$:
\STATE \quad \quad \quad \quad \quad $PtWsSum \leftarrow PtWsSum + DWsOutput[c][i][j] \times PtWsKernel[c][k]$
\STATE \quad \quad \quad \quad $finalOutput[i][j][k] \leftarrow PtWsSum$
\end{algorithmic}
%\caption{Converting CONV1D to DWSConv2D}
%\label{conv1D2conv2D}
\end{algorithm}

==> Algos/conv1DtoDWSconv2D.tex <==
\begin{algorithm}[H]
\label{algo:conv1D2conv2D}
\caption{Implementing Depth-wise Separable Convolution - DWSConv2D() using CONV1D ()}
\begin{algorithmic}[1]
\State \textbf{Function} DWSepConv2D($inputMatrix$, $DWsKernels$, $PtWsKernel$, $outputMatrix$):
\State \quad Initialize $DWsOutput$ with zero values, same shape as $inputMatrix$
\State \quad \# Depth-wise Separable (DWs) convolution
\State \quad \textbf{for} $c \leftarrow 0$ \textbf{to} $channels(inputMatrix) - 1$:
\State \quad \quad \# Apply 1D convolution along rows
\State \quad \quad \textbf{for} $i \leftarrow 0$ \textbf{to} $rows(inputMatrix[c]) - 1$:
\State \quad \quad \quad conv1D($inputMatrix[c][i, :]$, $DWsKernels[c][0, :]$, $DWsOutput[c][i, :]$)
\State \quad \quad \# Apply 1D convolution along columns
\State \quad \quad \textbf{for} $j \leftarrow 0$ \textbf{to} $cols(DWsOutput[c]) - 1$:
\State \quad \quad \quad conv1D($DWsOutput[c][:, j]$, $DWsKernels[c][:, 0]$, $DWsOutput[c][:, j]$)
\State \quad \# Point-wise (PtWs) convolution
\State \quad Initialize $finalOutput$ with zero values, with shape [rows($DWsOutput$), cols($DWsOutput$), channels($PtWsKernel$)]
\State \quad \textbf{for} $i \leftarrow 0$ \textbf{to} $rows(DWsOutput) - 1$:
\State \quad \quad \textbf{for} $j \leftarrow 0$ \textbf{to} $cols(DWsOutput) - 1$:
\State \quad \quad \quad \textbf{for} $k \leftarrow 0$ \textbf{to} $channels(PtWsKernel) - 1$:
\State \quad \quad \quad \quad Initialize $PtWsSum \leftarrow 0$
\State \quad \quad \quad \quad \textbf{for} $c \leftarrow 0$ \textbf{to} $channels(DWsOutput) - 1$:
\State \quad \quad \quad \quad \quad $PtWsSum \leftarrow PtWsSum + DWsOutput[c][i][j] \times PtWsKernel[c][k]$
\State \quad \quad \quad \quad $finalOutput[i][j][k] \leftarrow PtWsSum$
\State \quad \textbf{return} $finalOutput$
\end{algorithmic}
\end{algorithm}

==> Algos/uProfileCache.tex <==
\begin{algorithm}[H]
\caption{Measure Cache Characteristics Using Sequential Access}
\begin{algorithmic}[1]
\STATE Initialize a large array $A$ with size significantly larger than the expected cache size
\STATE Define $min\_size$ as the starting size of the data to test (e.g., 1KB)
\STATE Define $max\_size$ as the maximum size to test (e.g., size of $A$)
\STATE Define $step\_size$ to increment the test size (e.g., double the size each time)
\STATE Initialize $previous\_time$ to a high value
\FOR{size = $min\_size$ to $max\_size$ by $step\_size$}
    \STATE Access each element in $A[0:size-1]$ sequentially to ensure all data is loaded into cache
    \STATE Reset and start the high-resolution timer
    \STATE Access each element in $A[0:size-1]$ again to measure the cache hit time
    \STATE Record the time taken as $current\_time$
    \IF{$current\_time$ significantly greater than $previous\_time$}
        \STATE Print "Estimated cache size boundary at $size$ with time $current\_time$"
        \STATE Print "Cache hit time for size $size/2$ is $previous\_time$"
        \STATE Print "Memory hit time (cache miss) for size $size$ is $current\_time$"
        \STATE Break
    \ENDIF
    \STATE $previous\_time = current\_time$
\ENDFOR
\end{algorithmic}
\end{algorithm}


==> Algos/uProfileKernel.tex <==
\begin{algorithm}[H]
\caption{Profile Execution Time of Essential DNN Kernels}
\begin{algorithmic}[1]
\STATE Define the set of kernels to profile: GeMM, Convolution, ReLU, SoftMax
\STATE Initialize data structures for input, weights, and output appropriate for each kernel
\FOR{each kernel in the set}
    \STATE Prepare input data and weights specific to the kernel
    \STATE Warm up the system by running the kernel multiple times
    \STATE Reset and start the high-resolution timer
    \STATE Execute the kernel with the prepared data
    \STATE Stop the timer and record the execution time
    \STATE Store the execution time in a results array or dictionary
    \IF{kernel requires additional setup for different scenarios (e.g., different input sizes)}
        \STATE Repeat steps 4-8 for each scenario to measure how changes affect performance
    \ENDIF
    \STATE Output the execution times for each scenario or input size
\ENDFOR
\STATE Analyze the collected data to determine the performance bottlenecks and efficiency of each kernel
\end{algorithmic}
\end{algorithm}


==> figs/DynFitLoop.tex <==
\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black, fill=red!30]
\tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=orange!30]
\tikzstyle{decision} = [diamond, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=green!30]
\tikzstyle{arrow} = [thick,->,>=stealth]

\begin{tikzpicture}[node distance=2cm]

\node (start) [startstop] {Start};
\node (init) [process, below of=start] {Initialize DynAgent with EH profiles and HW characteristics};
\node (define) [process, below of=init] {Define energy budget $E_b$};
\node (initialize) [process, below of=define] {Initialize loop iteration parameters $l$};
\node (optimize) [process, below of=initialize] {OptimizeTaskQuanta()};
\node (forLayer) [process, below of=optimize, yshift=-1cm] {For each layer in the DNN};
\node (forLoop) [process, below of=forLayer, yshift=-1cm] {For each loop in the layer};
\node (estimate) [process, below of=forLoop] {Estimate energy $E_i$ using DynAgent};
\node (checkEnergy) [decision, below of=estimate, yshift=-1cm] {Is $E_i > E_b$?};
\node (adjust) [process, right of=checkEnergy, xshift=4cm] {Adjust $l_i$};
\node (checkConv) [process, below of=checkEnergy, yshift=-1cm] {Check Convergence};
\node (converged) [decision, below of=checkConv, yshift=-1cm] {Converged?};
\node (end) [startstop, below of=converged, yshift=-1cm] {End};

\draw [arrow] (start) -- (init);
\draw [arrow] (init) -- (define);
\draw [arrow] (define) -- (initialize);
\draw [arrow] (initialize) -- (optimize);
\draw [arrow] (optimize) -- (forLayer);
\draw [arrow] (forLayer) -- (forLoop);
\draw [arrow] (forLoop) -- (estimate);
\draw [arrow] (estimate) -- (checkEnergy);
\draw [arrow] (checkEnergy) -- node[anchor=east] {No} (checkConv);
\draw [arrow] (checkEnergy) -- node[anchor=south] {Yes} (adjust);
\draw [arrow] (adjust) |- (estimate);
\draw [arrow] (checkConv) -- (converged);
\draw [arrow] (converged) -- node[anchor=east] {No} (optimize);
\draw [arrow] (converged) -- node[anchor=west] {Yes} (end);

\label{Fig:DynFitLoop}
\caption{Write the Caption here}
\end{tikzpicture}

